Dropping Convexity for Faster Semi-definite Optimization

We study the minimization of a convex function $f(X)$ over the set of $n\times n$ positive semi-definite matrices, but when the problem is recast as $\min_U g(U) := f(UU^\top)$, with $U \in \mathbb{R}^{n \times r}$ and $r \leq n$. We study the performance of gradient descent on $g$---which we refer to as Factored Gradient Descent (FGD)---under standard assumptions on the original function $f$. We provide a rule for selecting the step size and, with this choice, show that the local convergence rate of FGD mirrors that of standard gradient descent on the original $f$: i.e., after $k$ steps, the error is $O(1/k)$ for smooth $f$, and exponentially small in $k$ when $f$ is (restricted) strongly convex. In addition, we provide a procedure to initialize FGD for (restricted) strongly convex objectives and when one only has access to $f$ via a first-order oracle; for several problem instances, such proper initialization leads to global convergence guarantees. FGD and similar procedures are widely used in practice for problems that can be posed as matrix factorization. To the best of our knowledge, this is the first paper to provide precise convergence rate guarantees for general convex functions under standard convex assumptions.

==> convergence.tex <==

\section{Convergence} \label{sec:convg}
In this section, we present the main convergence result for our scheme over the factor $U$ space. We first present the convergence guarantees under the general setting where $f$ satisfies the $(m, r)$-restricted strong convexity over $ \S_{+}^n $ and $U$ is restricted to be a $n\times r$ matrix, even though $\text{rank}(\Xo)$ can be larger than $r$. Later we present results for the special case when the optimum is exactly rank-$r$.%In particular, we show that, even though $f$ is non-convex in $U$, gradient descent motions converge linearly to $\Uo_r$, conditioned on each putative solution being close enough to $\Uo_r$.  As a by-product of this result, we discuss further ramifications of this theorem for special cases as $(i)$ $f$ satisfies strong convexity  over $ \S_{+}^n $ and $(ii)$ the optimum $\Xo$ is exactly rank-$r$ matrix. 

The following theorem characterizes the convergence rate of our scheme for $f$ that satisfy $(m, r)$-restricted strong convexity.

%We show that the error $\dist(\U, \Uo_r)$ decreases by a constant fraction in every iteration (thus ensuring linear convergence), when the current iterate $U$ is close to $\Uo$. The following theorem now precisely characterizes this convergence rate. 
 
\begin{theorem}[Convergence rate for rank-$r$ estimate of $\Xo$]\label{thm:convergence_main}
Let $\f: \S_{+}^n \rightarrow \R$ be a $M$-smooth and $(m, r)$-restricted strongly convex function, with restricted condition number $\kappa = \frac{M}{m}$. Let $\Xo$ be its minimum over the set of PSD matrices, such that $\|\Xo -\Xo_r\|_F \leq \frac{\sigma_r(\Xo)}{100 \kappa^{1.5}}\sqrt{\frac{\sigma_r(\Xo)}{\sigma_1(\Xo)}}$.  Let $\X^0=U^0(U^0)^\top$ be a rank-$r$ PSD matrix such that $ \dist(\U^0, \Uo_r)^2 \leq \rho \sigma_{r}(\Xo)$, for $\rho=\frac{1}{500 \kappa^2} \frac{\sigma_r(\Xo)}{\sigma_1(\Xo)}$. Let current iterate be $\U$ and $\X = \U\U^\top$. Let  $ \dist(\U, \Uo_r)^2 \leq \rho \sigma_{r}(\Xo)$ and set the step size as $\eta =\frac{1}{16 \, (M \norm{X^0 }_2 + \norm{\gradf(X^0)}_2) }$. Then, the new estimate $\Up= U -\eta \gradf(X) \cdot U$ satisfies
\begin{equation}
%\min_{R: R \in \mathcal{O}} \norm{\Up -\Uorr}_F^2 \leq \alpha \cdot \min_{R: R \in \mathcal{O}}\norm{\U - \Uorr}_F^2 + \beta \cdot ||\Xo -\Xo_r||_F^2,
\dist(\Up, \Uo_r)^2 \leq \alpha \cdot \dist(\U, \Uo_r)^2+ \beta \cdot ||\Xo -\Xo_r||_F^2, \label{conv:eq_00}
\end{equation}
where $\alpha = 1 -\frac{m \sigma_{r}(\Xo)}{208 (M||\Xo||_2 + \|\gradf(\Xo)\|_2)}$ and $\beta=  \frac{M}{24(M||\Xo||_2 + \|\gradf(\Xo)\|_2)}$. Further, $\Up$ satisfies \\$ \dist(\Up, \Uo_r)^2 \leq\rho \sigma_{r}(\Xo). $
 \end{theorem}

\noindent The theorem states that provided we $(i)$ choose the step size based on a point that is constant relative distance to $\Uo_r$, and $(ii)$ we start from such a point, gradient descent on $\U$ will converge linearly to a neighborhood of $\Uo_r$.
%In plain words, the above theorem shows that the proposed scheme exhibits fast convergence towards the vicinity of $\Xo_r$, whose radius depends on the spectral decay of the rank-$r$ approximation of $\Xo$. Moreover, using our step size selection and initialization, gradient descent motions -- on the factor $U$ space -- guarantee that every putative solution be close enough to $\Uo_r$. 

The above theorem immediately implies linear convergence rate for the setting where $f$ satisfies standard strong convexity with parameter $m$. This follows from observing that standard strong convexity implies restricted strong convexity for all values of rank $r$.
%\begin{corollary}[Strong convexity]\label{cor:strong}
%Let $\f: \S_{+}^n \rightarrow \R$ be a $M$-smooth and $m$-strongly convex function, with condition number $\kappa = \frac{M}{m}$. 
%Let $\Xo$ and $\X^0$ be defined as in Theorem \ref{thm:convergence_main}. 
%Then, the new estimate $\Up= U -\eta (\gradf(X)+\gradf(X)^\top)\cdot U$, for step size as in Theorem \ref{thm:convergence_main}, satisfies \eqref{conv:eq_00}
%where $\alpha$ and $\beta$ are defined in Theorem \ref{thm:convergence_main}. Further, $\Up$ satisfies $ \dist(\Up, \Uo_r)^2 \leq\rho \sigma_{r}(\Xo). $
% \end{corollary}

Now, when the optimum $\Xo$ is exactly rank-$r$ matrix, then our scheme indeed recovers it exactly with provable linear rate of convergence.
\begin{corollary}[Exact recovery of $\Xo$]\label{cor:exact}
Let $\f: \S_{+}^n \rightarrow \R$ be a $M$-smooth and $(m, r)$-restricted strongly convex function, with restricted condition number $\kappa = \frac{M}{m}$. Let $\Xo$ be its minimum over the set of PSD matrices, such that $rank(\Xo) =r$.  
Consider $X^0$ as in Theorem \ref{thm:convergence_main}. 
%Let $\X^0=U^0(U^0)^T$ be a rank-$r$ PSD matrix such that $ \dist(\U^0, \Uo)^2 \leq \rho \sigma_{r}(\Xo)$, for $\rho=\frac{1}{500 \kappa^2} \frac{\sigma_r(\Xo)}{\sigma_1(\Xo)}$. Let current iterate be $\U$ and $\X = \U\U^\top$. Let  $ \dist(\U, \Uo)^2 \leq \rho \sigma_{r}(\Xo)$. 
Then, under the assumption of Theorem \ref{thm:convergence_main}, we have %for step size as in Theorem \ref{thm:convergence_main}, we have
\begin{equation*}
%\min_{R: R \in \mathcal{O}} \norm{\Up -\Uorr}_F^2 \leq \alpha \min_{R: R \in \mathcal{O}}\norm{\U - \Uorr}_F^2 + \beta ||\Xo -\Xo_r||_F^2,
\dist(\Up, \Uo)^2 \leq \alpha \cdot \dist(\U, \Uo)^2,
\end{equation*}
where $\alpha = 1 -\frac{m \sigma_{r}(\Xo)}{208 (M||\Xo||_2 + \|\gradf(\Xo)\|_2)}$.\\% Further, $\Up$ satisfies $ \dist(\Up, \Uo)^2 \leq\rho \sigma_{r}(\Xo). $
 \end{corollary}

Further for $r =n$ we recover the exact case of semi-definite optimization.
\begin{remark}
\textit{By the results above, one can easily observe that the convergence rate factor $\alpha$, in contrast to standard convex gradient descent results, depends both on the condition number of $\Xo_r$ and $\|\gradf(\Xo)\|_2$, in addition to $\kappa$. This dependence is a result of the step size selection, which is different from standard step sizes, \textit{i.e.}, $\sfrac{1}{M}$ for standard gradient descent schemes. As discussed in Section~\ref{sec:algo}, this choice for $\eta$ is essential in order the algorithm not overshoot the optimum; we also refer the reader to Section~\ref{sec:discuss} for some discussion.}
% This is a consequence of doing gradient descent on $U$. We present some intuition about this dependence in Section~\ref{sec:discuss}.\\
\end{remark}

As a ramification of the above, notice that $\alpha$ depends only on the condition number of $\Xo_r$ and not that of $\Xo$. This suggests that, in settings where the optimum $\Xo$ has bad condition number -- and thus leads to slower convergence, it is indeed beneficial to restrict $U$ to be a $n \times r$ matrix and only search for a rank-$r$ approximation of the optimal solution, which leads to faster convergence rate in practice; see Figure \ref{fig:03}.

==> proof_factor_approx.tex <==
%\section{Proofs of Section~\ref{sec:rankr}}
\newcommand{\Uhp}{\plus{\hat{\U}}}
\newcommand{\Xhp}{\plus{\hat{\X}}}
\section{Proof of Theorem \ref{thm:convergence_main}}
We will use the following notation for the proof. $\tau(\Xor) =\frac{\sigma_{1}(\Xo)}{\sigma_{r}(\Xo)}$ denotes the condition number of $\Xo_r$. $Q_A$ denotes the basis of the column space of matrix $A$.

\begin{proof}[Proof of Theorem \ref{thm:convergence_main}.] Let $\U$ and $\Up$ be the current and the next iterate respectively. Without loss of generality assume $\gradf(\X)$ is a symmetric matrix (see Lemma~\ref{lem:grad}) and let $\Up =U -\eta \gradf(\X) U$.  Let $\weta =\frac{1}{16 (M||\X||_2 + \|\gradf(\X)Q_U Q_U^\top\|_2)}$. %Such a selection corresponds to a equivalent to the step size $\eta =\frac{1}{48 (M||\X^0||_2 + \|\gradf(\X^0)Q_{U^0} (Q_{U^0})^\top\|_2)}$ upto constants, as shown in Lemma~\ref{lem:stepsize}.\\

Let $\Uorr$ be such that $\Uorr (\Uorr)^\top =\Xo_r$ and $R_U$ denotes the optimal rotation that minimizes $||\U - \Uo_r R||_F$, through the rest of the proof. Using the algorithm's update rule, we obtain
\begin{align}
\dist(\Up, \Uo_r)^2 &\leq \norm{\Up -\Uorr }_F^2 \nonumber \\&= \norm{\Up -\U + \U -\Uorr }_F^2 \nonumber \\
&= \norm{\Up -\U}_F^2 + \norm{\U -\Uorr}_F^2 -2\ip{\Up -\U}{\Uorr -\U}, \label{proofs:eq_04}
\end{align}
which follows by adding and subtraction $\X$ and then expanding the square.

%\begin{remark}
%\textit{Throughout the proof, we use step size $\eta =\frac{1}{16 (M||\X||_2 + \|\gradf(\X)\|_2)}$. Such a selection corresponds to a larger step size, compared to the rule \eqref{eq:stepsize}. To see this, by the assumptions of the theorem, we have $\norm{\X -\Xo_r}_2 \leq \rho \norm{\Xo_r}_2$, for $\rho \leq \sfrac{1}{10 \tau(\Xo_r)}$.  Hence, based on Lemma~\ref{lem:init_ineq}, we get that, $\norm{\X^0_r}_2 \geq \sfrac{9}{11} \norm{\X}_2$ and $\norm{\gradf(\X^0_r)}_2 \geq \norm{\gradf(\X)}_2 - \sfrac{4}{9} M \norm{\X}_2$; this further leads to the inequality $\eta =\frac{1}{16 (M||\X||_2 + \|\gradf(\X)\|_2)} \geq \frac{1}{48(M||\X^0_r||_2 + \|\gradf(\X^0_r)\|_2)}.$ Thus, proving Theorem \ref{thm:lowrank_converge} for $\eta =\frac{1}{16 (M||\X||_2 + \|\gradf(\X)\|_2)}$ automatically applies for our step size selection.}
%\end{remark}

Now we will bound the individual terms on the right hand side of equation~\eqref{proofs:eq_04} and then combine them to get the convergence result. We will denote $\U - \Uorr$ with $\Delta$ for the rest of the proof. \\

\noindent{\bf Step I: Bounding term  $\ip{\U - \Up }{\U - \Uorr}$  in \eqref{proofs:eq_04}. } We first state the following key lemma that shows that the direction of update $\U - \Up $ is aligned with the direction $\U -\Uorr$; this further translates into lower bounding $\ip{\U - \Up }{\U - \Uorr}$ in \eqref{proofs:eq_04}. 
\begin{lemma}\label{lem:ip1r}
%Let $||\Delta||_F^2 \leq \rho \sigma_{r}(\Xo)$ for $\rho = \frac{1}{500 \kappa^2 \tau(\Xo_r)}$ and $\|\Xo -\Xo_r\|_F \leq \frac{\sigma_r(\Xo)}{100 \kappa^{1.5} \tau(\Xo_r)^{0.5}}$. 
Under the conditions of Theorem~\ref{thm:convergence_main},
\begin{align*}
\ip{\gradf(X) \U}{\U -\Uorr} \geq  \frac{3}{4} \weta  ||\gradf(X) U||_F^2 + \frac{m}{20} \cdot  \sigma_{r}(\Xo)  || \Delta||_F^2- \frac{M}{4}\norm{\Xo -\Xor}_F^2,
\end{align*}
where $\weta =\frac{1}{16 (M||\X||_2 + \|\gradf(\X)Q_U Q_U^\top\|_2)}$.
\end{lemma}

\paragraph{Step II: Combining bounds into \eqref{proofs:eq_04}.} Combining Lemma \ref{lem:ip1r} and \eqref{proofs:eq_04}, we get
\begin{align}
&\dist(\Up, \Uo_r)^2  \nonumber \\ &\leq \norm{\U -\Uorr}_F^2 +\eta^2 ||\gradf(X) \U ||_F^2- 2 \eta \left(   \frac{3}{4} \weta  ||\gradf(X) U||_F^2 + \frac{m}{20} \cdot  \sigma_{r}(\Xo)  || \Delta||_F^2 - \frac{M}{4}\norm{\Xo -\Xor}_F^2
 \right) \nonumber \\
&= \norm{\U -\Uorr}_F^2 +  \frac{\eta M}{2}\norm{\Xo -\Xor}_F^2 -\eta^2 \left( -||\gradf(X) \U||_F^2 + \frac{3}{2}\frac{\weta}{\eta} \norm{\gradf(X) \U}_F^2 \right) -\eta \left( \frac{m}{10} \cdot  \sigma_{r}(\Xo)  || \Delta||_F^2  \right) \nonumber \\
&\stackrel{(i)}{\leq}  \norm{\U -\Uorr}_F^2 + \frac{\eta M}{2}\norm{\Xo -\Xor}_F^2  -\eta \left(\frac{m}{10} \cdot  \sigma_{r}(\Xo)  || \Delta||_F^2  \right) \nonumber \\
&\stackrel{(ii)}{\leq}  \left(1 -\frac{\eta^*}{13} \cdot  m\sigma_{r}(\Xo) \right) \norm{\U -\Uorr}_F^2 +  \frac{ 6\eta^* }{9}M\norm{\Xo -\Xor}_F^2 \nonumber \\
&\stackrel{(iii)}{\leq}\left( 1 -\frac{m \sigma_{r}(\Xo)}{208 (M||\Xo||_2 + ||\gradf(\Xo)||_2)}\right)  \dist(\U , \Uo_r)^2 +  \frac{ M}{24(M||\Xo||_2 + ||\gradf(\Xo)||_2)}\norm{\Xo -\Xor}_F^2 ,
\end{align}
where $(i)$ and $(ii)$ follow from Lemma~\ref{lem:stepsize}. $(iii)$ follows from substituting $\eta^* =\frac{1}{16 (M||\Xo||_2 +  ||\gradf(\Xo)||_2)}$. \\

This proves the first part of the theorem. Now we will prove the second part where we show $\Up$ also satisfies the initialization condition. From the above equation we have,
\begin{align*}
\dist(\Up, \Uo_r)^2 &\leq \left( 1 -\frac{m \eta \sigma_{r}(\Xo)}{10} \right)  \dist(\U, \Uo_r)^2 +  \frac{\eta M}{2}\norm{\Xo -\Xor}_F^2 \nonumber \\
&\stackrel{(i)}{\leq}  \left( 1 -\frac{m \eta \sigma_{r}(\Xo)}{10} \right) \rho \sigma_r(\Xo) +  \frac{\eta M}{2}\frac{\sigma_r^2(\Xo)}{100^2 \kappa^3\tau(\Xo_r)} \\
&= \rho \sigma_r(\Xo) \left( 1 -\frac{\eta m \sigma_r(\Xo) }{10} + \frac{\eta m \sigma_r(\Xo)}{40}\right) \\
&\leq \rho \sigma_r(\Xo).
\end{align*}
$(i)$ follows from substituting the assumptions on $\dist(\U, \Uo_r)$ and $||\Xo -\Xo_r||_F$. 
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Lemma~\ref{lem:ip1r}}

Before we present proof of this lemma we prove another supporting lemma lower bounding $\ip{\gradf(\X)}{\X -\Xor}$.  %{\color{red} need more text}

\begin{lemma}\label{lem:ip2r}
Under the conditions of Theorem~\ref{thm:convergence_main},
\begin{align*}   \ip{\gradf(\X)}{\X-\Xor}  \geq 1.8 \weta ||\gradf(X) U||_F^2 +\frac{m}{2}\norm{\Xor -\X}_F^2 -\frac{M}{2}\|\Xo -\Xor\|_F^2,
\end{align*}
where  $\weta =\frac{1}{16 (M||\X||_2 + \|\gradf(\X)Q_U Q_U^\top\|_2)}$.
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{lem:ip2r}]

Now we will follow the standard proof technique of gradient descent convergence to lower bound $\ip{\gradf(\X)}{\X -\Xo_r}$ (see ~\cite{nesterov2004introductory} and \cite{agarwal2010fast}). %Note that while one can lower bound this quantity using restricted strong convexity directly, it leads to bad $\kappa$ dependence.
Let $\Uhp = U -\weta \gradf(\X) U$ and $\Xhp =\Uhp (\Uhp)^\top$. %and hence $\Xhp = X - \weta \gradf(\X)Q_U Q_U^\top U -\weta U Q_U Q_U^\top \gradf(\X) 

First using smoothness of $\f$ we get, \begin{align}\f(\X) &\geq \f(\Xhp) -\ip{\gradf(\X)}{\Xhp -\X} -\frac{M}{2} \norm{\Xhp -\X}_F^2 \nonumber \\ 
&\stackrel{(i)}{\geq} \f(\Xo) -\ip{\gradf(\X)}{\Xhp -\X} -\frac{M}{2} \norm{\Xhp -\X}_F^2 , \label{proofs1:eq_05}
 \end{align}
where $(i)$ follows from optimality of $\Xo$ and since $\Xhp$ is a feasible point for problem~\eqref{intro:eq_00}. 

Note that $\Xor$ is a PSD matrix and is feasible point. Using smoothness of $f$ we get,
\begin{align}
f(\Xor) &\leq f(\Xo) + \ip{\gradf(\Xo)}{\Xor -\Xo} + \frac{M}{2}\|\Xor -\Xo\|_F^2 \nonumber \\
&=f(\Xo)+ \frac{M}{2}\|\Xor -\Xo\|_F^2, \label{proofs1:eq_055}
\end{align}
since $\gradf(\Xo)\Xo =0$ by KKT conditions \cite{boyd2004convex}.

Now since $rank(\Xor)$ is $r$, using $(\rscm, r)$ restricted strong convexity of $\f$ we get, 
\begin{align} 
\f(\Xor) \geq \f(\X) +\ip{\gradf(\X)}{\Xor-\X} +\frac{m}{2}\norm{\Xor -\X}_F^2 .\label{proofs1:eq_06}
\end{align}
Combining equations~\eqref{proofs1:eq_05},~\eqref{proofs1:eq_055}, and~\eqref{proofs1:eq_06} we get, \begin{align} \ip{\gradf(\X)}{\X-\Xor} \geq  \ip{\gradf(\X)}{\X -\Xhp} -\frac{M}{2} \norm{\Xhp -\X}_F^2+\frac{m}{2}\norm{\Xor -\X}_F^2 -\frac{M}{2}\|\Xor -\Xo\|_F^2 \label{proofs1:eq_07} \end{align}

Now recall that \begin{align*}\Xhp &= X - \weta \gradf(X)X -  \weta X \gradf(X)+  \weta^2 \gradf(X)X \gradf(X) \\
&= X - \weta \left( \gradf(X)X\Lambda  + \Lambda^\top X \gradf(X) \right), \end{align*} where $\Lambda =I -\frac{\weta}{2} Q_{U} Q_{U}^\top \gradf(X)$. Notice that for step size $\weta$ considered $\Lambda \succ 0$,  $||\Lambda||_2 \leq  1+ \frac{1}{32}$ and $\sigma_{n}(\Lambda) \geq  1- \frac{1}{32}$.

Substituting above equation in~\eqref{proofs1:eq_07} gives,
\begin{align*}
 \ip{\gradf(\X)}{\X-\Xor} - \frac{m}{2}\norm{\Xo -\X}_F^2 &+\frac{M}{2}\|\Xor -\Xo\|_F^2  \\& \geq  \ip{\gradf(\X)}{ \weta(\gradf(X)X \Lambda + \Lambda^\top X \gradf(X)} -\frac{M}{2} \norm{ \weta \left( \gradf(X)X\Lambda  + \Lambda X \gradf(X) \right)}_F^2 \\
 &\stackrel{(i)}{\geq} 2\weta \trace( \gradf(X) \gradf(X)X \Lambda) -\frac{M}{2} 4 \weta^2 \norm{  \gradf(X)X\Lambda }_F^2 \\
 &\stackrel{(ii)}{\geq} 2 \weta \trace( \gradf(X) \gradf(X)X) \sigma_{\min}(\Lambda) -2 M \weta^2 \norm{  \gradf(X)U }_F^2 ||U||_2^2 ||\Lambda||_2^2 \\
 &\geq 2 \cdot \frac{31}{32} \weta ||\gradf(X) U||_F^2  -2 M \weta^2 \frac{33^2}{32^2} \norm{  \gradf(X)U }_F^2 ||U||_2^2  \\  
 &\geq  \frac{31}{16} \weta ||\gradf(X) U||_F^2 \left(1  - M \weta \frac{33^2}{32 \cdot 31}  ||X||_2 \right) \\
 &\stackrel{(iii)}{=} \frac{31}{16} \weta ||\gradf(X) U||_F^2 \left( 1  -  \frac{33^2}{32 \cdot 31 \cdot 16} \right)\\
 &\geq 1.8 \weta ||\gradf(X) U||_F^2.
 \end{align*}
$(i)$ follows from symmetry of $\gradf(X)$. $(ii)$ follows from Lemma~\ref{lem:lowtrace}. $(iii)$ follows from substituting $\weta$.
\end{proof}


%%%lem 1%%%%%
Now we are ready to present the proof of Lemma~\ref{lem:ip1r}

\begin{proof}[Proof of Lemma~\ref{lem:ip1r}]
We will use restricted strong convexity of $\f$ and closeness to optimum (small $||\Delta||_F$) to show this lower bound.

%\begin{align}
%\ip{\gradf(X) \U}{\U -\Uor} & \stackrel{(i)}{=} \ip{\gradf(X) Q_{U} Q_{U}^\top }{\X -\Uor \U^\top} \nonumber \\
%& \stackrel{(ii)}{=}  \frac{1}{2}\ip{\gradf(X) Q_{U} Q_{U}^\top }{\X -\Xo}  + \ip{\gradf(X) Q_{U} Q_{U}^\top }{\frac{1}{2}(\X + \Xo) -\Uor \U^\top} \nonumber \\
%&=  \frac{1}{2}\ip{\gradf(X) }{\X -\Xo}  + \frac{1}{2}\ip{\gradf(X) }{\Xo - \Xo Q_{U} Q_{U}^\top }   + \ip{\gradf(X) Q_{U} Q_{U}^\top }{\frac{1}{2}(\X + \Xo) -\Uor \U^\top}  \nonumber \\
%& =  \frac{1}{2}\ip{\gradf(X) }{\X -\Xo}  + \underbrace{\frac{1}{2}\ip{\gradf(X) }{\Xo Q_{U_{\perp}} Q_{U_{\perp}}^\top }}_\text{Err 1}   + \underbrace{\ip{\gradf(X) Q_{U} Q_{U}^\top }{\frac{1}{2}(\X + \Xo) -\Uor \U^\top}}_\text{Err 2} \label{proofs1:eq_09}
%\end{align}
%$(i)$ follows from $U = Q_{U} Q_{U}^\top U$. $(ii)$ follows by adding and subtracting $\Xo$. 

\begin{align}
\ip{\gradf(X) \U}{\U -\Uorr} &= \ip{\gradf(X) }{\X -\Uorr \U^\top} \nonumber \\
&=\frac{1}{2}\ip{\gradf(X) }{\X -\Xo_r}  + \ip{\gradf(X) }{\frac{1}{2}(\X + \Xo_r) -\Uorr \U^\top} \label{proofsr1:eq_09}
\end{align}
which follows by adding and subtracting $\Xo_r$.
By lemma~\ref{lem:ip2r} we can bound the first term in the above expression. Hence we will bound the second term now.

%\noindent {\bf Err1:}  
%\begin{align}
%\frac{1}{2}\ip{\gradf(X) }{\Xo Q_{U_{\perp}} Q_{U_{\perp}}^\top} &\stackrel{(i)}{=} \frac{1}{2} \trace\left((\gradf(X) -\gradf(\Xo) )\Xo Q_{U_{\perp}} Q_{U_{\perp}}^\top\right) \nonumber \\
%&
%\end{align}
%$(i)$ follows from $\gradf(\Xo)\Xo =0$.
%
%\noindent {\bf Err2:}  

First observe that \begin{align} \ip{\gradf(X) }{\frac{1}{2}(\X + \Xor) -\Uorr \U^\top} &= \ip{\gradf(X) }{\frac{1}{2} \left( (\U - \Uorr) \U^\top + \Uorr(\Uorr - \U)^\top \right)} \nonumber \\
&\stackrel{(i)}{=} \frac{1}{2}\ip{\gradf(X) }{  (\U - \Uorr) (\U - \Uorr)^\top} = \frac{1}{2}\ip{\gradf(X) }{ \Delta \Delta^\top}, \label{proofsr1:eq_10}
\end{align} where $(i)$ follows since $\gradf(X)$ is symmetric.


Now we can lower bound~\eqref{proofsr1:eq_10} as
 \begin{align}
\frac{1}{2}\ip{\gradf(X) }{ \Delta \Delta^\top} &\stackrel{(i)}{=} \frac{1}{2}\ip{Q_{\Delta} Q_{\Delta}^\top \gradf(\X) }{ \Delta \Delta^\top} \nonumber \\
&\geq - \frac{1}{2} \left|\trace\left(Q_{\Delta} Q_{\Delta}^\top \gradf(\X) \Delta \Delta^\top\right)\right| \nonumber \\ 
&\stackrel{(ii)}{\geq} -\frac{1}{2} || Q_{\Delta} Q_{\Delta}^\top \gradf(\X) ||_2 \trace( \Delta \Delta^\top)  \nonumber \\
&\stackrel{(iii)}{\geq} -\frac{1}{2} \left( ||Q_{U} Q_{U}^\top\gradf(\X)||_2+  ||Q_{\Uo_r} Q_{\Uo_r}^\top\gradf(X)||_2 \right)  || \Delta||_F^2 .   \label{proofsr1:eq_11}
%&\stackrel{(iv)}{\geq} -\frac{1}{2} \left(  ||Q_{U} Q_{U}^\top\gradf(\X)||_2 \rho \sigma_{\min}(\Xo) + ||Q_{\Uor} Q_{\Uor}^\top\gradf(X)||_2 || \Delta||_F^2  \right). \label{proofs1:eq_11}
\end{align}
Note that  $(i)$ follows from $\Delta =Q_{\Delta} Q_{\Delta}^\top \Delta$. $(ii)$ follows from $|\trace(AB)| \leq ||A||_2 \trace(B)$, for PSD matrix $B$ (Von Neumann's trace inequality~\cite{mirsky1975trace}). $(iii)$ follows from column space of $\Delta$, $\text{Span}(\Delta)$ is a subset of $\text{Span}(\U, \Uo_r)$, since $\Delta$ is a linear combination of $\U$ and $\Uorr$. % Finally $(iv)$ follows from the hypothesis of the Lemma. 

Now  we will bound the first term in equation~\eqref{proofsr1:eq_11}.
\begin{align}
& ||Q_{U} Q_{U}^\top\gradf(\X)||_2 \cdot || \Delta||_F^2 \nonumber \\&= \weta \cdot 16 \left(M||X||_2 +||Q_{U} Q_{U}^\top \gradf(X)||_2 \right) \cdot ||Q_{U} Q_{U}^\top\gradf(\X)||_2  || \Delta||_F^2  \nonumber \\
 &=  \weta \left( 16  M||X||_2 ||Q_{U} Q_{U}^\top\gradf(\X)||_2 \cdot || \Delta||_F^2 + 16 ||Q_{U} Q_{U}^\top\gradf(\X)||_2^2 \cdot  || \Delta||_F^2  \right) \nonumber \\
 &\stackrel{(i)}{\leq} \max \left\{\frac{16\cdot \weta}{5} \cdot M ||X||_2 \cdot m \sigma_r(\X)\cdot || \Delta||_F^2 ,~ \weta \cdot 16 \cdot 5 \kappa \tau(\X) ||Q_{U} Q_{U}^\top\gradf(\X)||_2^2 \cdot  || \Delta||_F^2 \right\} + 16\cdot \weta ||Q_{U} Q_{U}^\top\gradf(\X)||_2^2 \cdot  || \Delta||_F^2 \nonumber \\
 &\leq  \frac{16\cdot \weta}{5} M ||X||_2 \cdot m \sigma_{r}(\X)\cdot || \Delta||_F^2 +  \weta \cdot 16 \cdot 5 \kappa \tau(\X) ||Q_{U} Q_{U}^\top\gradf(\X)||_2^2 \cdot  || \Delta||_F^2  + 16 \cdot \weta ||Q_{U} Q_{U}^\top\gradf(\X)||_2^2 \cdot  || \Delta||_F^2 \nonumber \\
 &\stackrel{(ii)}{\leq}  \frac{1}{5}m \sigma_{r}(\X)\cdot || \Delta||_F^2 + (6 \kappa \tau(\Xo)+1) \cdot  16 \cdot \weta ||Q_{U} Q_{U}^\top\gradf(\X)||_2^2 \cdot \rho \sigma_{\min}(\Xo)  \nonumber \\
 &\stackrel{(iii)}{\leq}  \frac{1}{5} \cdot m \sigma_{r}(\X)\cdot || \Delta||_F^2 + 16 \cdot 7 \cdot \weta \cdot \kappa \tau(\Xo) \cdot ||\gradf(\X)U||_F^2 \cdot \frac{11\rho}{10}   \nonumber \\ 
 &\stackrel{(iv)}{\leq}  \frac{1}{5} \cdot m \sigma_r(\X)\cdot || \Delta||_F^2 + \frac{\weta}{4} \cdot ||\gradf(\X)U||_F^2,   \label{proofsr1:eq_12}
\end{align}
where $(i)$ follows from considering that one of the following cases hold: $||Q_{U} Q_{U}^\top\gradf(\X)||_2  \leq \frac{1}{5} \cdot m \sigma_{r}(\X)$ or $m \sigma_{r}(\X) \leq 5 ||Q_{U} Q_{U}^\top\gradf(\X)||_2$, $(ii)$ follows from substituting $\weta$, Lemma~\ref{lem:init_ineq} and bound on $|| \Delta||_F^2 \leq \rho \sigma_{\min}(\Xo) $, by the hypothesis of the lemma, $(iii)$ is due to $\sigma_{r}(\X)||Q_{U} Q_{U}^\top\gradf(X)||_2^2 \leq  ||U^\top\gradf(X)||_F^2$ and $\sigma_{r}(\Xo) \leq 1.1 \sigma_{r}(\X)$ from Lemma~\ref{lem:init_ineq}. Finally, $(iv)$ follows from substituting $\rho$ and using Lemma~\ref{lem:init_ineq}.

Now we will bound the second term in equation~\eqref{proofsr1:eq_11}.
\begin{align}
||Q_{\Uor} Q_{\Uor}^\top\gradf(X)||_2 || \Delta||_F^2 &\stackrel{(i)}{\leq}  ||\gradf(\X) -\gradf( \Xo) ||_2 || \Delta||_F^2 \nonumber \\
&\leq  ||\gradf(\X) -\gradf( \Xo) ||_F || \Delta||_F^2 \nonumber \\
&\stackrel{(ii)}{\leq} M (||\X -\Xo_r||_F +||\Xo -\Xo_r||_F)  || \Delta||_F^2 \nonumber \\
&\stackrel{(iii)}{\leq} M  (2+\sqrt{\rho}) ||\Uor||_2   || \Delta||_F \cdot || \Delta||_F^2 +  M||\Xo -\Xo_r||_F  || \Delta||_F^2  \nonumber \\
&\stackrel{(iv)}{\leq}  M  (2+\sqrt{\rho}) ||\Uor||_2  \frac{1}{\sqrt{500}\kappa \tau(\Uo_r)} \sigma_r(\Uo) \cdot || \Delta||_F^2  +    M||\Xo -\Xo_r||_F  || \Delta||_F^2  \nonumber \\
&\leq \frac{1}{10}m  \sigma_{r}(\Xo)   || \Delta||_F^2 +  M||\Xo -\Xo_r||_F  || \Delta||_F^2, \label{proofsr1:eq_13}
\end{align}
where $(i)$ follows from and $\gradf(\Xo)\Xo =0$, $(ii)$ is due to smoothness of $\f$ and $(iii)$ follows from Lemma~\ref{lem:ip4r}. Finally $(iv)$ follows from  $|| \Delta||_F^2 \leq \rho \sigma_{r}(\Xo)$ and substituting $\rho =  \frac{1}{500 \kappa^2 \tau(\Xor)}$.

Now from equations~\eqref{proofsr1:eq_09}, \eqref{proofsr1:eq_11}, \eqref{proofsr1:eq_12}, \eqref{proofsr1:eq_13}  and Lemma~\ref{lem:ip2r}  we get,
\begin{align*}
& \ip{\gradf(X) \U}{\U -\Uor}\\ &\geq \frac{9 }{10}\weta  ||\gradf(X) U||_F^2+\frac{m}{4}\norm{\X -\Xo}_F^2 - \frac{M}{4}\norm{\Xo -\Xor}_F^2 \\&- \frac{1}{2}\left(  \frac{\weta}{4 } ||\gradf(\X) U ||_F^2 + \frac{3}{10}  \cdot m\sigma_{r}(\Xo) \cdot || \Delta||_F^2   + M||\Xo -\Xo_r||_F  || \Delta||_F^2 \right) \nonumber \\
&\stackrel{(i)}{\geq}  \left(\frac{9}{10}- \frac{1}{8}\right) \cdot \weta  ||\gradf(X) U||_F^2 + \frac{m}{4}\left(\norm{\X -\Xo}_F^2 -  \frac{3}{5} \cdot \sigma_{r}(\Xo) \cdot || \Delta||_F^2 - \frac{1}{50} \cdot \sigma_{r}(\Xo) \cdot || \Delta||_F^2 \right)  - \frac{M}{4}\norm{\Xo -\Xor}_F^2 \nonumber \\
&\stackrel{(ii)}{\geq }  \frac{3}{4} \weta  ||\gradf(X) U||_F^2 + \frac{m}{20} \cdot  \sigma_{r}(\Xo)  || \Delta||_F^2 - \frac{M}{4}\norm{\Xo -\Xor}_F^2
\end{align*}
where $(i)$ follows from  $\|\Xo -\Xo_r\| \leq \frac{\sigma_r(\Xo)}{100 \kappa}$ and $(ii)$ follows from Lemma~\ref{lem:ip3r}.
\end{proof}

==> related.tex <==
\subsection{Related work}

\noindent \textbf{Convex approaches.} 
%We only briefly describe the work that revolves around solving convex instances of \eqref{intro:eq_00}. 
A significant volume of work has focused on solving the classic Semi-Definite Programming (SDP) formulation, where the objective $f$ (as well as any additional convex constraints) is assumed to be linear. There, interior point methods (IPMs) constitute a popular choice for small- and moderate-sized problems; see \cite{karmarkar1984new, alizadeh1995interior}. For a comprehensive treatment of this subject, see the excellent survey in \cite{monteiro2003first}.

Moving into high-dimensional settings, large scale SDPs pointed research towards first-order approaches, which are more computationally appealing. %due to their efficiency in high-dimensional settings. 
%; we only scratch the surface and refer the reader to references therein. 
For linear $f$, we note among others the work of \cite{wen2010alternating}, a provably convergent alternating direction augmented Lagrangian algorithm, and that of Helmberg and Rendl \cite{helmberg2000spectral}, where they develop an efficient first-order spectral bundle method for SDPs with the constant trace property; see also \cite{helmberg2014spectral} for extensions on this line of work. %, where subgradients of the dual function are used to build a cutting plane model of the objective function. 
In both cases, no convergence rate guarantees are provided;
%(randomized) multiplicative weights schemes \cite{garber2011approximating} and Frank-Wolfe type algorithms \cite{hazan2008sparse}. 
see also \cite{monteiro2003first}. For completeness, we also mention the work of \cite{burer2003semidefinite, fukuda2001exploiting, nakata2003exploiting, toh2004solving} on \emph{second-order} methods, that take advantage of data sparsity in order to handle high-dimensional SDPs in a more efficient way. However, it turns out that the amount of computations required per iteration is comparable to that of log-barrier IPMs \cite{monteiro2003first}. % for an excellent survey and references therein. 
%Convex problems of such form have a well-understood structure and, hence, high accuracy solutions can be obtained within polynomial time and with superlinear convergence rate by using the celebrated IPMs \cite{karmarkar1984new, }; see also \cite{gonzaga1992path} and references therein. Representative implementations include but not restricted to primal-dual approaches \cite{alizadeh1998primal, vandenberghe1995primal} and projective methods \cite{karmarkar1984new, nesterov1994interior}. 

Standard SDPs have also found application in the field of combinatorial optimization; there, in most cases, even an rough approximation via SDP is sufficiently better than exhaustive combinatorial algorithms. Goemans and Williamson \cite{goemans1995improved} were the first to propose the use of SDPs in approximating graph \textsc{Max Cut}, where a near-optimum solution can be found in polynomial-time complexity. \cite{klein1996efficient} propose an alternative approach for solving \textsc{Max Cut} and \textsc{Graph Coloring} instances, where SDPs are transformed into eigenvalue problems. Then, power method iterations lead to $\varepsilon$-approximate solutions; however, the resulting running-time dependence on $\varepsilon$ is worse, compared to standard IPMs. Arora, Hazan and Kale in \cite{arora2005fast} derive an algorithm to approximate SDPs, as a hybrid of the Multiplicative Weights Update method and \cite{vaidya1989new}, improving upon existing algorithms for graph partitioning, computational biology and metric embedding problems.\footnote{The algorithm in \cite{arora2005fast} shows significant computational gains over standard IPMs per iteration, due to requiring only a power method calculation per iteration (versus a Cholesky factorization per iteration, in the latter case). However, the polynomial dependence on the accuracy parameter $\tfrac{1}{\varepsilon}$ is worse, compared to IPMs. Improvements upon this matter can be found in \cite{arora2007combinatorial} where a primal-dual Multiplicative Weights Update scheme is proposed.}

Extending to generic convex $f$ cases, \cite{nesterov1988general, nesterov1989self} have shown how IPMs can be generalized to solve instances of \eqref{intro:eq_00}, via the notion of self-concordance; see also \cite{lee2012proximal, trandihn15a} for a more recent line of work. %Despite their superlinear convergence rate, such methods are usually based on Newton second-order updates and, thus, suffer from the curse-of-dimensionality and can be mostly used for small-sized problems.
Within the class of first-order methods, approaches for nonlinear convex $f$ include, among others, projected and proximal gradient descent methods \cite{nesterov2004introductory, trandihn15a, jiang2012inexact}, (smoothed) dual ascent methods \cite{nesterov2007smoothing}, as well as Frank-Wolfe algorithm variants \cite{jaggi2011convex}. As a concluding remark, we note that all these schemes, while efficient even for large-scale problems, often require extra heavy calculations, such as eigenvalue decompositions, in order to remain within the feasible set.\\

\noindent \textbf{Burer \& Monteiro factorization and related work.}
Burer and Monteiro \cite{burer2003nonlinear, burer2005local} popularized the idea of solving classic SDPs by representing the solution as a product of two factor matrices. The main idea in such representation is to remove the positive semi-definite constraint by directly embedding it into the objective. While the problem becomes non-convex, Burer and Monteiro propose a method-of-multiplier type of algorithm which iteratively updates the factors in an alternating fashion. For linear objective $f$, they establish convergence guarantees to the optimum but do not provide convergence rates. 

Specialized algorithms -- for objectives beyond the linear case -- that utilize such factorization include matrix completion solvers \cite{jain2013low}, non-negative matrix factorization schemes \cite{lee2001algorithms}, phase retrieval methods \cite{netrapalli2013phase, candes2014solving, candes2015phase} and sparse PCA algorithms \cite{laue2012hybrid}. Restricted to the case of matrix completion, \cite{jain2013low} shows linear convergence (with $O(\log(1/\varepsilon))$ steps) in solving \eqref{intro:eq_01}. Tu et al. \cite{tu2015low} study the problem of recovering a low-rank PSD matrix from linear measurements and propose \textit{Procrustes Flow}, a local search heuristic, that solve the problem at hand under standard restricted isometry assumptions on the linear map; for a similar recent discussion on the subject, we refer to \cite{zheng2015convergent}. Both these approaches admit linear convergence to the optimal solution by employing a careful initialization step. Nevertheless, both \cite{tu2015low} and \cite{zheng2015convergent} only apply to simple quadratic loss objectives and not to generic convex functions $f$. 

For generic smooth convex functions, Hazan in \cite{hazan2008sparse} proposes \textsc{SparseApproxSDP} algorithm,\footnote{Sparsity here corresponds to low-rankness of the solution, as in the Cholesky factorization representation. Moreover, inspired by Quantum State Tomography applications \cite{aaronson2007learnability}, \textsc{SparseApproxSDP} can also handle constant trace constraints, in addition to PSD ones. } a generalization of the Frank-Wolfe algorithm for the vector case \cite{clarkson2010coresets}, where putative solutions are refined by rank-1 approximations of the gradient. At the $r$-th iteration, \textsc{SparseApproxSDP} is guaranteed to compute a $\tfrac{1}{r}$-approximate solution, with rank at most $r$, \textit{i.e.}, achieves a sublinear $O\left(\tfrac{1}{\varepsilon}\right)$ convergence rate. Application of these ideas in machine learning tasks can be found in \cite{shalev2011large}. Based on \textsc{SparseApproxSDP} algorithm, \cite{laue2012hybrid} further introduces ``de-bias'' steps in order to optimize parameters in \textsc{SparseApproxSDP} and do local refinements of putative solutions via L-BFGS steps. Nevertheless, the resulting convergence rate is still sublinear. % framework, where the rank-1 update is followed by a nonlinear improvement of the current solution using the L-BFGS algorithm. 

At the time of submission, we became aware of the work of Chen and Wainwright \cite{chen2015fast}. There, the authors propose a fast, first-order optimization framework for the problem \eqref{intro:eq_00}, where the same parameterization technique is used to efficiently accommodate the PSD constraint in optimization.\footnote{In this work, the authors further assume orthogonality of columns in $\U$.} Withal, the proposed algorithmic solution can accommodate extra constraints on $\X$.\footnote{Though, additional constraints should satisfy the $\Xo$-\textit{faithfulness} property: a constraint set on $\U$, say $\mathcal{U}$, is faithful if for each $\U \in \mathcal{U}$, that is within some bounded radius from optimal point, we are guaranteed that the closest (in the Euclidean sense) rotation of $\Uo$ lies within $\mathcal{U}$.} Their results are of the same flavor with ours: under proper assumptions\footnote{The set of assumptions listed in \cite{chen2015fast} must hold only locally and include, apart from $\Xo$-faithfulness, local descent, local Lipschitz and local smoothness conditions. These conditions less standard than the global assumptions of the current work and one needs to validate they are satisfied for each problem separately. However, \cite{chen2015fast} presents a rather wide range of diverse settings and applications where these conditions are indeed satisfied in practice.}, one can prove global convergence with $O(1/\varepsilon)$ or  $O(\log(1/\varepsilon))$ rate and for $f$ instances that fail to be locally convex or are globally concave, even.

Finally, for completeness, we also mention optimization over the Grassmannian manifold that admits tailored solvers~\cite{edelman1998geometry}; see \cite{keshavan2010matrix, boumal2014optimization} for applications in matrix completion and references therein. \cite{journee2010low} presents a second-order method for \eqref{intro:eq_00}, based on manifold optimization over the set of all equivalence classes of the form $\{UR ~:~ R \in \R^{r \times r}, R^\top R = I_{r \times r}, ~U \in \R^{n \times r}\}$. The proposed algorithm can additional accommodate constant trace constraints and enjoys monotonic decrease of the objective function (in contrast to \cite{burer2003nonlinear, burer2005local}), featuring quadratic local convergence. However, it requires performing an full eigenvalue decomposition or matrix inversion per iteration, which is computationally expensive for large-scale settings.\footnote{In particular, the proposed scheme in \cite{journee2010low} looks for the smallest eigenvalue of a matrix per iteration. For this task and for general matrices $\X$, an non-exhaustive list of approaches include full eigen-value decomposition, inversion followed by power iteration and, power iteration and deflation. The complexity of all the above is equivalent, up to constants.}

Table \ref{table:algo_comp_summary} summarizes the discussion above for the case of matrix factorization techniques.

\begin{table*}[!htb]
\centering
\begin{small}
\begin{tabular}{c c c c c c c c c}
  \toprule
  Reference & & Oracle & & Conv. rate & & SVD & & Setting \\ 
  \cmidrule{1-1} \cmidrule{3-3} \cmidrule{5-5} \cmidrule{7-7} \cmidrule{9-9} 
	  \cite{burer2003nonlinear, burer2005local} & & $\nabla f$ & & - & & None & & SDP \\
      \cite{jain2013low} & & $\nabla f$ & &  $\log(\sfrac{1}{\varepsilon})$ & & Init. (once) $/$ top-$r$ & & MC, MS \\
      \cite{tu2015low} & & $\nabla f$ & &  $\log(\sfrac{1}{\varepsilon})$ & & Init. (multiple) $/$ top-$r$ & & MS, PT \\
      \cite{zheng2015convergent} & & $\nabla f$  & & $\log(\sfrac{1}{\varepsilon})$ & & Init. (once) $/$ top-$r$ & & MS, PT \\
      \cite{shalev2011large} & & $\nabla f$ & & - & & Per iter. $/$ top-$1$ & & Smooth $f$ \\
      \cite{hazan2008sparse} & & $\nabla f$  & & $\sfrac{1}{\varepsilon}$ & & Per iter. $/$ top-$1$ & & Smooth $f$ \\      
      \cite{laue2012hybrid} & & $\nabla f$  & & $\sfrac{1}{\varepsilon}$ & & Per iter. $/$ top-$1$ & & Smooth $f$ \\
      \cite{chen2015fast} & & $\nabla f$  & & $\sfrac{1}{\varepsilon}$ & & Init. (once) $/$ top-$r^{\dagger}$ & & (Locally) Lipschitz $f$ \\
      \cite{chen2015fast} & & $\nabla f$  & & $\log(\sfrac{1}{\varepsilon})$ & & Init. (once) $/$ top-$r^{\dagger}$  & & (Locally) smooth $f$ \\
      \cite{journee2010low} & & $\nabla^2 f$  & & $\log\log(\sfrac{1}{\varepsilon})$ & & Per iter. $/$ full & & Smooth $f$ \\      
  \midrule
      This work & & $\nabla f$  & & $\log(\sfrac{1}{\varepsilon})$ & & Init. (twice) $/$ top-$1$ & & Smooth, RSC $f$ \\      
  \bottomrule
\end{tabular}
\end{small}
\caption{Summary of selected results on solving variants of \eqref{intro:eq_00} via matrix factorization. ``Oracle" indicates the order of information that is utilized: $\nabla f$ (gradient information, first-order) and $\nabla^2 f$ (Hessian information, second order). ``Convergence rate" omits Big-Oh notation and describes the number of iterations required to achieve $\epsilon$ accuracy. ``SVD" indicates the existence of a singular value decomposition operation in the algorithms: ``Init. (once)" signifies that one SVD is performed only at the initialization step, ``Init. (multiple)" signifies that \emph{multiple} SVDs are performed only at the initialization step while ``Per iter.'' indicates that SVD is performed per iteration of the algorithm; ``top-$r$" means that a rank-$r$ decomposition is performed, while ``full'' means that a full SVD decomposition is performed (\textit{i.e.}, can be a function of the ambient dimension). For the case of \cite{chen2015fast}, top-$r^{\dagger}$ corresponds to the initialization procedure used in most examples considered. MC = matrix complextion, MS = matrix sensing, PT = phase retrieval, RSC = restricted strongly convex.} \label{table:algo_comp_summary} 
\end{table*}

\begin{table*}[!htb]
\centering
\begin{small}
\begin{tabular}{c c c c c c c}
  \toprule
  Reference & & Convergence & & $\dist\left(\Up, \Uo\right)^2 \leq \alpha \cdot \dist\left(\U, \Uo \right)^2$ & & $\dist\left(\U^0, \Uo\right) \leq \cdots$ \\ 
	  \cmidrule{1-1} \cmidrule{3-3} \cmidrule{5-5} \cmidrule{7-7}
	  \cite{tu2015low} & & Linear & & $\alpha = 1 - \tfrac{c_1}{\tau(\Uo_r)^4}$ & & $\tfrac{1}{4}\sigma_r(\Uo_r)$ \\
      \cite{zheng2015convergent} & & Linear & & $\alpha = 1 - \tfrac{c_2}{\tau(\Uo_r) \cdot r}$  & & $\sqrt{\tfrac{3}{16}} \cdot \sigma_r(\Uo_r)$ \\
      \cite{chen2015fast} & & Linear & & $\alpha = 1 - \tfrac{c_3}{\tau(\Uo_r)^6}$  & & $\left(1 - \tau\right) \cdot \sigma_r(\Uo_r)$ \\      
  \midrule
      This work & & Linear & & $\alpha = ?$  & & $?$ \\  
  \bottomrule
\end{tabular}
\end{small}
\caption{Summary of selected results on solving variants of \eqref{intro:eq_00} via matrix factorization. } \label{table:convergence_comp_summary} 
\end{table*}


%``top-$i$ comp." indicates that a $i$-rank SVD is performed at the $i$-th iteration, for $i = 1, \dots, r$, 

%{\bf Burer Monteriro ~\cite{burer2003nonlinear, burer2005local}} popularized the idea of solving classic SDP\rq{}s( instances of \eqref{intro:eq_00}) by representing the solution as product of two factor matrices. While the problem becomes non-convex, Burer and Monteiro propose a method-of-multiplier type of algorithm. 

%\paragraph{Other approaches.} \textcolor{magenta}{not sure whether we need to explain or somehow say "Other approaches include + citations"} 
%
%A different line of work includes optimization over the Grassmanian manifold~\citep{edelman1998geometry}; also see \cite{boumal2014low} for applications in matrix completion over the Grassmanian manifold and references therein. % Finally, \cite{} propose Random Conic Pursuit, an efficient algorithm that minimizes generic $f$ iteratively using sampling techniques repeatedly randomly sampling
%%a PSD matrix and optimizing over the random two-dimensional subcone given by this matrix and


%\noindent {\bf BM}
%
%
%
%\noindent {\bf ALS}
%
%Factorization machine, MC, NMF, Sparse PCA etc..
%
%\noindent {\bf Other}
%
%SGD
